RAPID: Efficient Retrieval-Augmented Long Text Generation with Writing Planning and Information Discovery

Generating knowledge-intensive and comprehensive long texts, such as encyclopedia articles, remains significant challenges for Large Language Models. It requires not only the precise integration of facts but also the maintenance of thematic coherence throughout the article. Existing methods, such as direct generation and multi-agent discussion, often struggle with issues like hallucinations, topic incoherence, and significant latency. To address these challenges, we propose RAPID, an efficient retrieval-augmented long text generation framework. RAPID consists of three main modules: (1) Retrieval-augmented preliminary outline generation to reduce hallucinations, (2) Attribute-constrained search for efficient information discovery, (3) Plan-guided article generation for enhanced coherence. Extensive experiments on our newly compiled benchmark dataset, FreshWiki-2024, demonstrate that RAPID significantly outperforms state-of-the-art methods across a wide range of evaluation metrics (e.g. long-text generation, outline quality, latency, etc). Our work provides a robust and efficient solution to the challenges of automated long-text generation.

==> tables/human_rubric.tex <==
\begin{table*}
\centering
\scriptsize
\begin{tblr}{
    cell{24}{1} = {r=2}{},
    cell{41}{1} = {r=2}{},
    hline{1,2,9,10,17,18,26,27,34,35,43} = {-}{0.08em},
    colspec = {ll}
}
Criteria Description & \textbf{Interest Level} \\ 
Score 1 Description & Not engaging at all; no attempt to capture the reader’s attention. \\ 
Score 2 Description & Slightly engaging with rare moments that capture attention. \\ 
Score 3 Description & Fairly engaging with a basic narrative but lacking depth. \\ 
Score 4 Description & Moderately engaging with several interesting points. \\ 
Score 5 Description & Quite engaging with a well-structured narrative and noteworthy points that frequently capture and retain attention. \\ 
Score 6 Description & Very engaging with a compelling narrative that captures and mostly retains attention. \\ 
Score 7 Description & Exceptionally engaging throughout, with a compelling narrative that consistently stimulates interest. \\ 

Criteria Description& \textbf{Coherence and Organization} \\ 
Score 1 Description &Disorganized; lacks logical structure and coherence. \\ 
Score 2 Description & Poor organization; some structure is evident but very weak. \\ 
Score 3 Description & Fairly organized; a basic structure is present but not consistently followed. \\ 
Score 4 Description & Organized; a clear structure is mostly followed with some lapses in coherence. \\ 
Score 5 Description & Good organization; a clear structure with minor lapses in coherence. \\ 
Score 6 Description & Very well-organized; a logical structure with transitions that effectively guide the reader. \\ 
Score 7 Description & Excellently organized; the article is logically structured with seamless transitions and a clear argument. \\ 

Criteria Description & \textbf{Relevance and Focus} \\ 
Score 1 Description & Off-topic; the content does not align with the headline or core subject. \\ 
Score 2 Description & Mostly off-topic with some relevant points. \\ 
Score 3 Description & Somewhat on topic but with several digressions; the core subject is evident but not consistently adhered to. \\ 
Score 4 Description & Generally on topic, despite a few unrelated details. \\ 
Score 5 Description & Mostly on topic and focused; the narrative has a consistent relevance to the core subject with infrequent digressions. \\ 
Score 6 Description & Highly relevant with a focused narrative and purpose. \\ 
Score 7 Description & Exceptionally focused and entirely on topic; the article is tightly centered on the subject, with every piece of information contributing to a compre-\\
& hensive understanding of the topic. \\ 

Criteria Description & \textbf{Broad Coverage} \\ 
Score 1 Description & Severely lacking; offers little to no coverage of the topic’s primary aspects, resulting in a very narrow perspective. \\ 
Score 2 Description & Minimal coverage; addresses only a small selection of the topic’s main aspects, with significant omissions. \\ 
Score 3 Description & Partial coverage; includes some of the topic’s main aspects but misses others, resulting in an incomplete portrayal. \\ 
Score 4 Description & Acceptable breadth; covers most main aspects, though it may stray into minor unnecessary details or overlook some relevant points. \\ 
Score 5 Description & Good coverage; achieves broad coverage of the topic, hitting on all major points with minimal extraneous information. \\ 
Score 6 Description & Comprehensive; provides thorough coverage of all significant aspects of the topic, with a well-balanced focus. \\ 
Score 7 Description & Exemplary in breadth; delivers outstanding coverage, thoroughly detailing all crucial aspects of the topic without including irrelevant information. \\ 

Criteria Description & \textbf{Verifiability} \\ 
Score 1 Description & No supporting evidence; claims are unsubstantiated. \\ 
Score 2 Description & Rarely supported with evidence; many claims are unsubstantiated. \\ 
Score 3 Description & Inconsistently verified; some claims are supported; evidence is occasionally provided. \\ 
Score 4 Description & Generally verified; claims are usually supported with evidence; however, there might be a few instances where verification is lacking \\ 
Score 5 Description & Well-supported; claims are very well supported with credible evidence, and instances of unsupported claims are rare. \\ 
Score 6 Description & Very well-supported; almost every claim is substantiated with credible evidence, showing a high level of thorough verification. \\ 
Score 7 Description & Exemplary verification; each claim is supported by robust, credible evidence from authoritative sources, reflecting strict adherence to the no origi- \\
&nal research policy. \\ 
         
\end{tblr}
\caption{Scoring rubrics for Human Evaluation}
\label{table:human_eval_rubric}
\end{table*}
